Hyperbolic Learning with Synthetic Captions for Open-World Detection

Open-world detection poses significant challenges, as it requires the detection of any object using either object class labels or free-form texts. Existing related works often use large-scale manual annotated caption datasets for training, which are extremely expensive to collect. Instead, we propose to transfer knowledge from vision-language models (VLMs) to enrich the open-vocabulary descriptions automatically. Specifically, we bootstrap dense synthetic captions using pre-trained VLMs to provide rich descriptions on different regions in images, and incorporate these captions to train a novel detector that generalizes to novel concepts. To mitigate the noise caused by hallucination in synthetic captions, we also propose a novel hyperbolic vision-language learning approach to impose a hierarchy between visual and caption embeddings. We call our detector ``HyperLearner''. We conduct extensive experiments on a wide variety of open-world detection benchmarks (COCO, LVIS, Object Detection in the Wild, RefCOCO) and our results show that our model consistently outperforms existing state-of-the-art methods, such as GLIP, GLIPv2 and Grounding DINO, when using the same backbone.

==> Table/COCO.tex <==
\begin{table*}[!t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|c|c|c|ccc}
   \toprule
    Method & Detection Backbone & Architecture & Text Model & AP\textsubscript{novel} & AP\textsubscript{base} & AP\textsubscript{all} \\
    \hline
    ViLD & R50-FPN & Faster R-CNN  & CLIP  & 27.6 & 59.5 & 51.2 \\
    BARON\textsuperscript{1} & CLIP  & Faster R-CNN & CLIP  & 34.0 & 60.4 & 53.5 \\
    OV-DETR & R50-C4  & DeformableDETR  & CLIP   & 29.4 & 61.0 & 52.7 \\
    CORA & R50-C4 & DAB-DETR & CLIP  & 35.1 & 35.5 & 35.4 \\
    OVR-CNN & R50-C4 & Faster R-CNN & BERT   & 22.8 & 46.0 & 39.9 \\ 
    Detic & R50-C4 & Faster R-CNN & CLIP   & 27.8 & 51.1 & 45.0 \\
    BARON\textsuperscript{2} & CLIP  &  Faster R-CNN & CLIP &  33.1 & 54.8 & 49.1 \\
    PB-OVD	& R50-FPN & Mask R-CNN & CLIP  &  30.8  & 46.1 & 42.1 \\
    \textbf{Ours} & R50-FPN & CenterNet-v2 & CLIP   & 33.8 & \textbf{61.1} & \textbf{54.0} \\ 
    \hline
        RegionCLIP & RN50x4-C4 & Faster R-CNN & CLIP  & 39.3  & \textbf{61.6} & \textbf{55.7} \\
        CORA^{+} & R50x4-C4 & DAB-DETR & CLIP & 43.1 & 60.9 & 51.7 \\
        BARON^{\dagger} & R50-C4 & Faster R-CNN & CLIP & 42.7 & 54.9 & 51.7 \\
        \textbf{Ours}^{\dagger} & R50-FPN & CenterNet-v2 & CLIP & \textbf{45.1} &  55.4 & 52.7 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Experimental Results on COCO Benchmark}
    \label{tab:OVCOCO}
\end{table*}

==> Table/OVLVIS.tex <==
\begin{table}[!t]
    \centering
    \resizebox{0.49\textwidth}{!}{%
    \begin{tabular}{l|c|c|c}
  \toprule
       \multirow{2}{*}{Method} & \multirow{2}{*}{\makecell{Pretraining Data}} &  \multicolumn{2}{c}{\makecell{LVIS minival} }  \\ 
    & & AP & APr/APc/APf \\ 
    \hline
    MDETR~\cite{kamath2021mdetr} & GoldG, RefCOCO & 24.2 & 20.9 / 24.9 / 24.3 \\ 
    DETCLIP-T~\cite{yao2022detclip} & O365 & 28.8 &  26.0 / 28.0 / 30.0 \\
    GLIP-T (C)~\cite{li2022grounded}  & O365, GoldG & 24.9 & 17.7 / 19.5 / 31.0 \\ 
    GLIP-T~\cite{li2022grounded} & O365, GoldG, Cap4M & 26.0  & 20.8 / 21.4 / 31.0 \\ 
    Grounding-DINO-T~\cite{liu2023grounding}  & O365, GoldG & 25.6& 14.4 / 19.6 / \textbf{32.2} \\ 
    Grounding-DINO-T~\cite{liu2023grounding} & O365, GoldG, Cap4M & \textbf{27.4} & \textbf{20.8 / 21.4 / 31.0} \\ 
    \hline
    Ours & O365 & 25.5 & 25.9 / 27.5 / 23.7 \\
    Ours & O365, GoldG & \textbf{31.3} & \textbf{30.7 / 32.6 / 30.3} \\
    \bottomrule
    \end{tabular}
    }
    \vskip -0.5em
    \caption{Experimental results on LVIS benchmark}
    \vskip -0.5em
\label{tab:OVLVIS}
\end{table}


